Staggercast: Demand-Side Management for ISPs

The continuing expansion of Internet media consumption has increased traffic volumes, and hence congestion, on access links. In response, both mobile and wireline ISPs must either increase capacity or perform traffic engineering over existing resources. Unfortunately, provisioning timescales are long, the process is costly, and single-homing means operators cannot balance across the last mile. Inspired by energy and transport networks, we propose demand-side management of users to reduce the impact caused by consumption patterns out-pacing that of edge network provision. By directly affecting user behaviour through a range of incentives, our techniques enable resource management over shorter timescales than is possible in conventional networks. Using survey data from 100 participants we explore the feasibility of introducing the principles of demand-side management in today's networks.

==> characterizing.tex <==
\section{The Case for DSM}
\label{sec:data-chars}

Before we discuss different techniques for DSM in this context, we must first
establish evidence that DSM is applicable at all. We begin by inspecting traces taken from the BBC iPlayer catch-up service. These traces consist of a 25\% of all video and radio requests between July 3--16, 2010. Altogether the traces consist of streaming times and episode information for 6,696,057 requests from 1,806,829 users, a 25\% sample of all usage. Figure~\ref{fig:diurnal_pattern} presents the daily access patterns of users. As is well understood, it can be seen that demand varies significantly over time. To support these viewing styles, capacity must either be wasted or exhausted.


\subsection{Elasticity in Peak Demand}
                                                 
To examine the potential for staggering peak demand, we use the two
datasets detailed below.




\begin{figure}[t!]
  \includegraphics[width=\columnwidth,height=1.5in]
                  {figs/diurnal_pattern.pdf}
\caption{\label{fig:diurnal_pattern}Diurnal pattern of normalized request
  volumes shows that there is a well defined peak. Staggering the redundant
  requests during the peak period would result in better network utilisation.}
\end{figure}




\paragraph{Elasticity Analysis}
Using these datasets, we explore the elasticity of home network traffic;
in other words the extent to which it can be shifted. Elasticity is difficult to
measure precisely as it depends fundamentally on the user's desires, needs,
mood, etc., but anecdotal evidence suggests that most users' video
consumption is somewhat elastic: Some would be prepared to watch different
content, and many would be prepared to watch it at a different time,
for example, by pre-fetching it during off-peak times or simply
delaying viewing for a period of time.

Given this anecdotal evidence, we use video traffic as our case-study
shiftable traffic type in the rest of this paper. \fref{fig:timeseries} shows
the average traffic utilization for a household in the BISmark testbed, per
hour of the day over the course of June 2012. The timeseries shows the diurnal
patterns for all unanonymized traffic from the household,
%(i.e.,~all traffic that is either in the Alexa top 100 or in our set of whitelisted domains)
as well as the fraction of that unanonymized traffic that we deem to be
``shiftable''. We classify as shiftable any long-lived traffic flows to
domains of content distribution networks, or any long-lived flows that
originate from a device that is known to be primarily a streaming device
(e.g.,~a Roku set-top box) as this is likely to be video traffic.\footnote{We
assume all traffic identified as video streams could be time-shifted; but due
as some are live, e.g.,~sporting events, demand for these will
be less elastic than others. The analysis we present here is simply
to illustrate there is a significant amount of streaming traffic
during peak hours, some of which could be shifted.} This illustrative example,
coupled with evidence from previous studies~\cite{sandvine}, suggests that
there is a non-negligible fraction of traffic that users might be willing to
delay, given appropriate incentives.

Extending this analysis, \fref{fig:diurnal_pattern} complements this
view from the home to show the diurnal variation in request volumes from the
BBC iPlayer traces. Unlike the BISmark traces, \emph{all} of this traffic is
potentially shiftable, as this data excludes live events. The clear temporal
variation in request patterns indicates that staggering users across time
could certainly decrease peak use.

\subsection{Techniques for Internet DSM}

There are many possible mechanisms for applying demand-side management in the
Internet. We identify three main categories here, but we do not claim that
this is an exhaustive list. In \S\ref{sec:managing} we investigate mechanisms
implementing the first two techniques.

\one~{\bf Space shifting}. In-network caching is a technique that has been
widely proposed and evaluated (e.g.,~\cite{network-caching}), but is
typically deployed in the form of CDNs (requiring content to be pre-loaded,
and paid for by the provider), and does little to reduce load in the access
network. In the right context, this technique could provide a
significant incentive to users to shift demand off their ISP's access network.
Interest in content from providers such as the BBC is likely to be
geographically correlated based on demographic and content (e.g.,~football
matches involving a local team). Thus, it may also be possible to use local
overlapping in-home WiFi to redirect content requests directly between users,
without needing to request it over the access network.

\two~{\bf Time shifting}. One obvious cause of high peak loads is that user
demand is correlated in time: people usually want to watch content as soon as
it is available, and even if downloaded for offline consumption, automatic
downloaders will often fetch the content as soon as possible. One way the
content provider could encourage---or even enforce---time shifting is to
introduce advertising into the content stream: although this might slightly
increase total resource consumed by a peak, it could have the effect of
spreading the initial load of heavily loaded content servers. By offsetting
consumption patterns, even for live events, this might also have beneficial
effects on the energy network by de-synchronising start, break and finish
times for viewers. Alternatively, the ISP could encourage time shifting by
granting different, and potentially higher, guaranteed user download
bandwidths at different times.

\three~{\bf Content shifting}. Finally, depending on the type of content and
the actual elasticity of user demand, it may even be possible to shift users'
\emph{preferences} in the specifics of what they consume. For example, content
provider directory services could encourage particular content to be
downloaded for offline viewing rather than immediate streaming; or could
encourage subscription to ``programs like $x$'' as a way to manipulate user
choices (to become more easily cacheable). Applied to such a large population,
these approaches could have a significant effect overall even without
affecting every single individual. In the most extreme case, users could even
be offered alternative content items at request-time (e.g.,~nearby cached
items) in an attempt to mitigate peak traffic loads. This latter point seems
to show strong potential considering the power of
recommendations~\cite{Davidson:2010}. Such techniques could perhaps be
implemented by having the ISP re-write HTML in the access network to alter
content recommendations or front page suggestions, as directed by the content
provider.

\subsection{Impact of Internet DSM}

Bringing users' elasticity of demand into consideration could significantly
affect the overall network architecture and market structure. For instance,
ISPs might sell cache space at the edge to content providers, who can then
encourage users to shift content viewing patterns to make more effective use
of caching, (e.g.,~reducing advertising in free content, or offering paid
content at a lower price to users who shift their requests to a less busy
period or to locally cached content).

Alternately, ISPs might directly engage their customers, offering incentives
such as higher guaranteed rates in return for shifting demand. Those ISPs
well-provisioned enough to have excess capacity at peak times might also
\emph{encourage} their users to make content requests during peak times to
fill caches. Access to these locally cached copies could then be offered to
other ISPs or the content provider in a \emph{spot market}, enabling requests
from geographically neighbouring users connected to other ISPs to be fulfilled
by the cached copy. Thus, as well as relieving peak hour congestion, bandwidth
scarcity in the access network can be turned into a source of profit for both
access ISPs and users.




%% (3) introduction of two-sided market between ISP and content provider, via specific mechanism of caching at the far edges of the network (ie., not just in-network caching, but in-aggregation-point caching)

%% (4) Addition of a market between ISPs: neighbours who are on different ISPs can move/share content from one ISP to another.



%Whether or not a system could actually exploit this redundancy depends
%on the temporal and spatial scope of redundant requests. A larger
%aggregate would increase the chances of a locating a user with a cached
%copy, but larger groups of users may also be spread over a wider
%geographic area (or across different access networks); in such cases,
%requesting the content from a peer would not relieve access-link
%congestion, although the ISP could still garner benefits from shifting
%demands to off-peak times.  



%This is a problem of aggregating users along the distribution tree. On
%the one hand, it is easy to achieve savings at the root and decrease
%the burden of the content provider using a peer-to-peer approach,
%simply by redirecting a content request to another user who has
%recently accessed the same item. Indeed, commercial applications such
%as Spotify~\cite{kreitz2010spotify} and PPLive~\cite{huang08pplive}
%have shown that this strategy can be successful. However, this may not
%ncessarily translate into lower traffic for ISPs as users might be
%paired with other users who are ``far away'' from each other in a
%network sense. On the other hand, there is usually little sharing
%possible at the leaf level, behind users sharing the same IP.  






==> implications.tex <==

Finally, the architecture potentially creates new markets to design,
explore, and study: 
%for example, encouraging users to
%retrieve nearby low cost (cached) content through incentives and
%discounts creates a second market between the content provider and the
%ISP. Ultimately, ISPs might sell cache space to content qproviders who
%would wish to encourage users to view their content, who would then have
%incentives to view this cached content at a discount. 
%DSM is a radical departure from conventional ISP business models
%which assume little or no dialog between ISPs and users.  Staggercast
%thus significantly affects the overall network architecture and market
%structure. 
For instance, ISPs might sell storage space at the edge to
content providers, who can then encourage users to shift content viewing
patterns to make more effective use of caching, (e.g.,~reducing
advertising in free content, or offering paid content at a lower
price). Undoubtedly, our proposal raises many questions (and potential
concerns) regarding net neutrality, particularly when considering
strategies involving content shifting and manipulation of user
interfaces and recommendations to affect demand.  In many cases, the
user might be completely unaware that they are participating in DSM,
which also raises potential legal and ethical questions relating to
disclosure.

Staggercast plants a stake in the network neutrality landscape (or,
perhaps more accurately, it plants a stake in the heart of network
neutrality). Yet, we believe that such trends are inevitable, which
makes it imperative that we explore more flexible ways to price content
and traffic, lest we miss an opportunity to improve network efficiency.
In some cases, users may in fact benefit by paying for (and receiving
compensation for) services that more accurately reflect the value of
delivering bits over the network.  Ultimately, by making the costs of
delivering content more transparent through flexible pricing, the
efficiency of network markets may improve.  As one example, ISPs
well-provisioned enough to have excess capacity at peak times might
\emph{encourage} their users to make content requests. Such excess
capacity could thus be used to fill local caches, which users of
\emph{other} ISPs could pay to access (e.g., as a ``spot market'' for
caches). Thus, in addition relieving peak-time congestion, bandwidth
scarcity in the access network can be turned into a source of profit for
both access ISPs and users.

We acknowledge that such an approach is inherently risky: it puts
network neutrality to rest; it has considerable security. privacy, and
ethical implications; and users themselves may not indulge in the
pricing mechanisms that might improve network efficiency if the
interfaces do not make prices and options transparent and easy to
understand.  Yet, we believe that these challenges---and the potential
positive benefits of a successful DSM architecture---are precisely what
makes this research area worth exploring further.

%\subsection{DSM: User rights and requirements}
%\nn{Need to discuss invasion into rights and requirements of user - DSM should only be with user consent and participation. And what happens with partial participation? Also today's networks are optimized for higher download bandwidth. Ultimately, DSM, esp with the caching at the edge, may require upload participation from users, e.g., if enabled by ISP-friendly P2P. Networks may need to be provisioned for this.}
%\gareth{Yep, this could perhaps go into a ``privacy and user rights'' section?}
%\mort{this seems to be to be somewhat covered above -- what else do you want to add here?}


==> managing.tex <==
\section{\bf\large \emph{Staggercast}, A Strawman}
\label{sec:managing} 

We next present a simple evaluation of a strawman system, \emph{Staggercast}, which uses edge caching to encourage users to shift consumption during peak hours. 



\subsection{System Outline}


As in today's network, all users have the option to retrieve content from the original content distribution network. However, Staggercast offers users the opportunity to either delay their requests, or re-direct them to a nearby cache. Staggercast places caches in two places: \one~in the network, at routers or the Broadband Remote Access Server (BRAS); and \two~in users' home networks, so that they may be accessible by other users within WiFi range. This ensures that time-shifted requests are automatically fetched into the cache without user involvement.

When a user initiates a high-volume download (e.g.,~of streaming media, though other high-volume downloads can be treated similarly) during peak hours, the system prompts the user to find out whether they would be willing to delay their original request, or change it to a different content item that is less costly for the network to access. Drawing inspiration from previous work~\cite{prabhakar2009:netecon}, in return for either option the user receives points which might ultimately translate into benefits such as discounts.


If the user opts to defer the download to a later time, Staggercast aborts the current download request and then attempts to fulfil it at a later time. Specifically, the user selects a new access time\footnote{Different access times may well result in content ultimately being fetched from different points.} after which the request is automatically pre-fetched into a nearby cache for the user to access. In contrast, if the user agrees to change their request to a less costly one, the new item is simply retrieved immediately from the nearby cache. Ideally, Staggercast caches would already have the desired content at the desired time and could immediately satisfy the user with little effect on the network.




There are many aspects of this design that warrant exploration. Foremost among these, the effectiveness of such a system depends on appropriately rewarding users for shifting their traffic demands, which presupposes that they are willing to shift their traffic demands in the first place. As described in~\S\ref{sec:summary}, we are planning to test this assumption via user studies in real-world deployments. In this paper, we simply evaluate the {\em potential} for content reuse that a system like Staggercast could offer, based on the locality of demands for shiftable traffic that could exist if the system were deployed.






